Counting Everyday Objects in Everyday Scenes

We are interested in counting the number of instances of object classes in natural, everyday images. Previous counting approaches tackle the problem in restricted domains such as counting pedestrians in surveillance videos. Counts can also be estimated from outputs of other vision tasks like object detection. In this work, we build dedicated models for counting designed to tackle the large variance in counts, appearances, and scales of objects found in natural scenes. Our approach is inspired by the phenomenon of subitizing - the ability of humans to make quick assessments of counts given a perceptual signal, for small count values. Given a natural scene, we employ a divide and conquer strategy while incorporating context across the scene to adapt the subitizing idea to counting. Our approach offers consistent improvements over numerous baseline approaches for counting on the PASCAL VOC 2007 and COCO datasets. Subsequently, we study how counting can be used to improve object detection. We then show a proof of concept application of our counting methods to the task of Visual Question Answering, by studying the `how many?' questions in the VQA and COCO-QA datasets.

==> sections/discussion.tex <==
\begin{comment}
The three methods presented in the paper \glance{}, \detect{} and \sub{} have interesting connections to work in psychology on how children \emph{learn} to count. It has been found that children are good at subitizing~\cite{yunsubitizing} to counts of smaller values ($\approx 4$) from a \glance{} of the image. The subitizing method doesnt work as well for higher counts, thus children learn to count by enumerating and accumulating counts one by one. Our \sub{} method is a middle ground between explicit enumeration in \detect{} and implicit count estimates in \glance{}.
\TODO{For standard datasets such as PASCAL, these counts may be trivially extracted from the detection annotations. However, for future dataset collection efforts, annotating counts is a lot easier than annotating bounding boxes for all instances.}
\end{comment}

%An interesting outcome of our experiments is in the performance of detection finetuned features for tasks like counting, especially when used in the \sub{} model. One tends to think of classification features as defacto choices when approaching any scene understanding task. Our results, however put things in perspective. There are some situations (especially when dealing with local image regions) when using a detector finetuned feature might be beneficial. 
%Our work opens up interesting avenues for future work to focus upon. For example, one could count with object completeness constraints in the \seq{} method to further improve the performace. It would also be interesting to explore label based context for counting. That is, if we knew that four chairs are present, is a table also likely to be there? 

\begin{comment}
Our work opens up interesting avenues for future work to focus upon. It would be interesting to explore cardinality based loss functions to produce integer counts for the \glance{} and \sub{} methods. It would also be interesting to count with object completeness constraints in the \sub{} method. That is, we can use context that says that if 0.3 fraction of an object is in some box, an adjacent box should probably have the object as well. It would also be interesting to explore label based context for counting. That is, if we knew that four chairs are present, is a table also likely to be there? 
\end{comment}

\begin{comment}
Link to how children learn to count. Detection vs subitizing.
Connecting Subitizing Detection and Associative subitizing
\begin{itemize}
\item  "how many soccer players are wearing red uniforms"
\end{itemize}
\begin{itemize}
\item We can view associative subitizing as a spectrum covering detection to subitizing
\item In a view of detection for counting, we restrict our counts outputs to binary, and accumulate counts across boxes
\item Subitizing on the other hand is a special case of associative subitizing where the number of regions is 1 (the whole image)
\item One can think of other ways to explore the continuum, perhaps use \emph{counting proposals} similar to how people do object proposals as future work
\end{itemize}
Other approaches for counting
associative subitizing - similar to density based approaches but at some appropriate granularity
\begin{itemize}
\item It would also be interesting to explore cardinality based loss functions to produce integer counts
\item It would be interesting to count with geometric/object completeness constraints -- for fractional ground truth take the completeness of objects into account
\item Counting by exploiting context (if it doesn't end up working for us)
\item It would be interesting to fine-tune the CNN features and contrast if the learnt representations for counting are different
\item learnt to recognize parts in images?
\item One can also think of counting as a weak supervision, to learn object detectors. Previous work has explored this idea on MNIST images
\end{itemize}

\end{comment}
